Analyzing the Data from X-ray Polarimeters with Stokes Parameters

X-ray polarimetry promises to deliver unique information about the geometry of the inner accretion flow of astrophysical black holes and the nature of matter and electromagnetism in and around neutron stars. In this paper, we discuss the possibility to use Stokes parameters - a commonly used tool in radio, infrared, and optical polarimetry - to analyze the data from X-ray polarimeters such as scattering polarimeters and photoelectric effect polarimeters, which measure the linear polarization of the detected X-rays. Based on the azimuthal scattering angle (in the case of a scattering polarimeter) or the azimuthal component of the angle of the electron ejection (in the case of a photoelectric effect polarimeter), the Stokes parameters can be calculated for each event recorded in the detector. Owing to the additive nature of Stokes parameters, the analysis reduces to adding the Stokes parameters of the individual events and subtracting the Stokes parameters characterizing the background (if present). The main strength of this kind of analysis is that the errors on the Stokes parameters can be computed easily and are well behaved - in stark contrast of the errors on the polarization fraction and polarization direction. We demonstrate the power of the Stokes analysis by deriving several useful formulae, e.g. the expected error on the polarization fraction and polarization direction for a detection of $N_S$ signal and $N_{BG}$ background events, the optimal observation times of the signal and background regions in the presence of non-negligible background contamination of the signal, and the minimum detectable polarization (MDP) that can be achieved when following this prescription.

==> uncertainties.tex <==
\section{Uncertainties of Polarization Measurements}\label{sec:uncertainties}
When employing a sine fit of the azimuth distribution in order to determine the polarization parameters $p$ and~$\chi$, authors typically assume that $Q$ and $U$ are normally distributed and uncorrelated~\citep{vinokur_m_1965, vaillancourt_je_2006, weisskopf_mc_2006}:
\begin{multline}
  P(Q,U)=\\
    \frac{1}{2\pi\sigma^2}\exp\left[-\frac{(Q-\langle Q\rangle)^{2}+(U-\langle U\rangle)^{2}}{2\sigma^2}\right],
\end{multline}
or 
\begin{multline}
  P(p,\chi|p_0,\chi_0)=\\
    \frac{p}{2\pi\sigma^2}\exp\left[-\frac{p_0^2  + p^2 - 2pp_0\cos\bigl(2(\chi-\chi_0)\bigr)}{2\sigma^2}\right]
\label{probabilitydistributionequation}
\end{multline}
Assuming Poissonian statistics, $N_\mathrm{bin}$ bins in azimuth and on average $\bar{n}$ events per bin, one arrives at~\cite{weisskopf_mc_2006,krawczynski_h_2011a}:
\begin{multline}\label{eq:weisskopf_prob}
  P(p,\chi|p_0,\chi_0) = \frac{p \, \mu^2 N_\mathrm{bin} \, \bar{n}}{4\pi} \times \\
    \exp\left[-\frac{\mu^2 N_\mathrm{bin} \, \bar{n}}{4}(p^2 + p_0^2 - 2pp_0\cos\bigl(2(\chi-\chi_0)\bigr)\right].
\end{multline}

We take a slightly different approach and derive the uncertainties of the Stokes Parameters $Q$ and $U$, as well as their correlation, from the definitions given in the previous section.
In analogy to equations~\eqref{eq:q_expectation} and~\eqref{eq:u_expectation} one finds
\begin{equation}
  \langle q^2\rangle = \langle u^2\rangle = \frac{1}{2}.
\end{equation}
Using $\Var(q)=\langle q^2\rangle - \langle q\rangle^2$ (and the same for $u$) and the definitions~\eqref{eq:total-stokes-Q} and~\eqref{eq:total-stokes-U} error propagation yields
\begin{subequations}\begin{align}
  \sigma_Q^2 &= \frac{W_2}{4}\bigl(2-p_0^2\mu^2\cos^2(2\chi_0)\bigr)
\intertext{and}
  \sigma_U^2 &= \frac{W_2}{4}\bigl(2-p_0^2\mu^2\sin^2(2\chi_0)\bigr)
\end{align}\end{subequations}
with
\begin{equation}
  W_2 = \sum_{k=1}^N w_k^2.
\end{equation}

In order to compute the correlation of $Q$ and $U$, we first note that
\begin{equation}
  \langle qu\rangle = \int\limits_0^{2\pi}\cos(2\alpha)\sin(2\alpha)f_\alpha(\alpha) \, \dd\alpha = 0,
\end{equation}
and thus
\begin{equation}
  \cov(q,u) = -\frac{p_0^2\mu^2}{8}\sin(4\chi_0).
\end{equation}
Because $q_i$ and $u_j$ for different photons are clearly uncorrelated, i.\,e.\ $\cov(q_i, u_j) = \delta_{ij}\cov(q,u)$, the covariance of $Q$ and $U$ is
\begin{equation}
  \cov(Q, U) = -\frac{W_2p_0^2\mu^2}{8}\sin(4\chi_0).
\end{equation}
Then, the linear correlation coefficient is
\begin{equation}\begin{split}
  \rho(Q, U) &= \frac{\cov(Q,U)}{\sigma_Q\sigma_U} \\
    &= -\frac{p_0^2\mu^2 \sin(4\chi_0)}{\sqrt{16 - 8p_0^2\mu^2 + p_0^4\mu^4\sin^2(4\chi_0)}}.
\end{split}\end{equation}
which is independent of $N$.
Figure~\ref{fig:QU_correlation_chi} shows this correlation as a function of true polarization angle $\chi_0$.
The fact that this correlation depends on the true polarization angle is by itself interesting since the reference direction on the sky for $\chi_0$ is arbitrary.
The correlation vanishes when $\chi_0$ is a multiple of $45\degree$, i.\,e.\ when $\langle Q\rangle = 0$ or $\langle U\rangle = 0$. 
The maximum value for $\chi_0 = -22.5\degree$ and $p_0=\mu=1$ is
\begin{equation}
  \rho_\text{max} = \frac{1}{3}.
\end{equation}

\begin{figure}
  \centering
  \includegraphics[width=\figurewidth]{QU_correlation_chi}
  \caption{Correlation of the Stokes Parameters $Q$ and $U$ as a function of true polarization angle $\chi_0$, assuming a polarization fraction and modulation factor of $p_0=\mu=1$.}
  \label{fig:QU_correlation_chi}
\end{figure}

Assuming a bivariate normal distribution for $Q$ and $U$,
\begin{multline}
  P_{QU}(Q, U) = \frac{1}{2\pi\sigma_Q\sigma_U\sqrt{1-\rho^2}} \times \\
    \exp\left[-\frac{1}{2(1-\rho^2)}\left(\frac{(Q-\langle Q\rangle)^2}{\sigma_Q^2} + \frac{(U-\langle U\rangle)^2}{\sigma_U^2} \right.\right.\\
       \left.\left.-\frac{2\rho(Q - \langle Q\rangle)(U - \langle U\rangle)}{\sigma_Q\sigma_U}\right)\right],
\end{multline}
where $\rho \equiv \rho(Q,U)$, one finds for the polarization fraction and direction:
\begin{multline}\label{eq:pchi_prob}
  P(p,\chi|p_0,\chi_0) = \frac{\sqrt{I^2/W_2}\,p\,\mu^2}{2\pi\sigma} \times \\
    \exp\biggl[-\frac{\mu^2}{4\sigma^2} \biggl\{p_0^2+p^2 - 2pp_0\cos\bigl(2(\chi-\chi_0)\bigr) \\
    - \frac{p^2p_0^2\mu^2}{2}\sin^2\bigl(2(\chi-\chi_0)\bigr)\biggr\}\biggr],
\end{multline}
where $\sigma$ is defined as
\begin{equation}\label{eq:pchi_sigma}
  \sigma = \sqrt{\frac{W_2}{I^2}\left(1 - \frac{p_0^2\mu^2}{2}\right)}.
\end{equation}
This is an approximation since (a)~$Q^2 + U^2 \leq N^2$ and, therefore, $Q$ and $U$ cannot be normally distributed for large values of $Q$ and $U$, and (b)~the correlation between $Q$ and $U$ is not exactly linear but follows a circle with radius~$I/2$.
The former is not an issue because $\langle Q^2 + U^2\rangle \leq I^2/2$.
Additionally, $\sigma_Q,\sigma_U \propto \sqrt{W_2} \ll \pi I$ for large $N$, so that the linear approximation of the correlation is good.\fkcomment{How does this argument change when weights are ${>}1$?}

The biggest difference between Eq.~\eqref{eq:pchi_prob} and Eq.~\eqref{eq:weisskopf_prob} is the third term in the exponent.
It accounts for the fact that the standard deviations of~$Q$ and~$U$ differ for large~$p_0$.
Furthermore, $\sigma$ defined in Eq.~\eqref{eq:pchi_sigma} contains a second order correction in~$p_0$ accounting for reduced variance at large~$p_0$.

\fkcomment{Question to Henric: these calculations are pretty detailed. Should we reduce their description?}
